Polymer size in dilute solutions in the good-solvent regime

We determine the density expansion of the radius of gyration, of the hydrodynamic radius, and of the end-to-end distance for a monodisperse polymer solution in good-solvent conditions. We consider the scaling limit (large degree of polymerization), including the leading scaling corrections. Using the expected large-concentration behavior, we extrapolate these low-density expansions outside the dilute regime, obtaining a prediction for the radii for any concentration in the semidilute region. For the radius of gyration, comparison with field-theoretical predictions shows that the relative error should be at most 5% in the limit of very large polymer concentrations.

==> paperraggi-ref.tex <==

\bibitem{deGennes-72}
de Gennes,~P.G. {\em Phys. Lett.} {\bf 1972}, {\em 38A}, 339.

\bibitem{deGennes-79}
de Gennes,~P.G. {\em Scaling Concepts in Polymer Physics;} \/
Cornell University Press: Ithaca, NY, 1979.

\bibitem{Freed-87}
Freed,~K.F. {\em Renormalization Group Theory of Macromolecules;} \/
Wiley: New York, 1987.

\bibitem{dCJ-book}
des Cloizeaux,~J.; Jannink,~G.
{\em Polymers in Solution: Their Modelling and Structure;} \/
Clarendon: Oxford, 1990.

\bibitem{Schaefer-99}
Sch\"afer,~L. {\em Excluded Volume Effects in Polymer Solutions;} \/
Springer Verlag: Berlin, 1999.

\bibitem{bestnu}
At present the most accurate estimates of $\nu$ are  
$\nu = 0.58758 \pm 0.00007$ (Ref.~\CITE{BN-97}),
$\nu = 0.5874 \pm 0.0002$ [Prellberg,~T. {\em J. Phys. A} {\bf 2001}, {\em 34}, L599.], $\nu = 0.58765 \pm 0.00020$ [Hsu,~H.-P.; Nadler,~W.; Grassberger,~P.
{\em Macromolecules} {\bf 2004}, {\em 37}, 4658.].
For an extensive list of results, see Ref.~\CITE{PV-review}.

\bibitem{DE-book}
Doi, Edwards {\bf perfezionare}

\bibitem{BN-97}
Belohorec,~P.; Nickel,~B.G. 
``Accurate universal and two-parameter model results
from a Monte-Carlo renormalization group study,''
Guelph University report (1997), unpublished.

\bibitem{footPsi}
The interpenetration radius is determined from the low-density behavior of
the osmotic pressure $\Pi$. If $\Pi/(R T\rho) = 1/M + B_2 \rho$ ($M$ is 
the molar mass of the polymer, $\rho$ the ponderal concentration, and 
$T$ the absolute temperature),
$\Psi = 2 (4\pi)^{-3/2} M^2 B_2 R^{-3}_g/N_A$, where $N_A$ is the 
Avogradro number. 

\bibitem{CMP-viriale}
Caracciolo,~S.; Mognetti,~B.M.; Pelissetto,~A. ``Virial coefficients and osmotic pressure in polymer solutions in good-solvent conditions,'' 
available at {\tt www.arxiv.org/abs/cond-mat/0605535}.

\bibitem{DRSK-02}
D\"unweg,~B.; Reith,~D.; Steinhauser,~M.;  Kremer,~K. 
{\em J. Chem. Phys.} {\bf 2002}, {\em 117}, 914.

\bibitem{DJ-72}
Domb,~C.; Joyce,~G.S. {\em J. Phys. C} {\bf 1972}, {\em 5}, 956.

\bibitem{Lal}
Lal,~M. {\em Molec. Phys.} {\bf 1969}, {\em 17}, 57.
%%CITATION = MOPHA,17,57;%%
 
\bibitem{MacDonald}
MacDonald,~B.; Jan,~N.; Hunter,~D.L.; Steinitz,~M.O.
{\em J. Phys. A: Math. Gen.} {\bf 1985}, {\em 18}, 2627.
%%CITATION = JPAGB,18,2627;%%
 
\bibitem{Madras-Sokal}
Madras,~N.; Sokal,~A.D. {\em J. Stat. Phys.} {\bf 1988}, {\em 50}, 109.
%%CITATION = JSTPB,50,109;%%    

\bibitem{Sokal-95b}
Sokal,~A.D. in {\em Monte Carlo and Molecular Dynamics Simulations
in Polymer Science, edited by K. Binder;} \/
Oxford Univ. Press: Oxford, 1995.

\bibitem{Kennedy-02}
Kennedy,~T. {\em J. Stat. Phys.} {\bf 2002}, {\em 106}, 407.

\bibitem{CPP-94}
Caracciolo,~S.; Parisi,~G.; Pelissetto,~A.
{\em J. Stat. Phys.} {\bf 1994}, {\em 77}, 519.

\bibitem{LMS-95}
Li,~B.; Madras,~N.; Sokal,~A.D. {\em J. Stat. Phys.} {\bf 1995}, {\em 80}, 661.

\bibitem{PH-05}
Pelissetto,~A.; Hansen,~J.-P.
{\em J. Chem. Phys.} {\bf 2005}, {\em 122}, 134904.

\bibitem{PV-review}
Pelissetto,~A.; Vicari,~E.
{\em Phys. Rept.} {\bf 2002}, {\em 368}, 549.

\bibitem{GSS-97}
Grassberger,~P.; Sutter,~P.; Sch\"afer,~L.
{\em J. Phys. A} {\bf 1997}, 7039.

\bibitem{footnote-Sg}
See Eq.~(18.11) of Ref.~\CITE{Schaefer-99}. Note that $\hat{s}$ is related 
to our variable $c \hat{R}_g^3$ by 
$\Phi_p = 4\pi c \hat{R}_g^3/3 = 1.169 \hat{s}$.

\bibitem{Nickel-91}
Nickel,~B.G. {\em Macromolecules} {\bf 1991}, {\em 24}, 1358.   

\bibitem{ON-83}
Ohta,~T.; Nakanishi,~A.
{\em J. Phys. A}  {\bf 1983}, {\em 16}, 4155.

\bibitem{Freed-83}
Freed,~K.F.
{\em J. Chem. Phys.} {\bf 1983}, {\em 79}, 6357.

\bibitem{Schaefer-84}
Sch\"afer,~L. {\em Macromolecules} {\bf 1984}, {\em 17}, 1357.

\bibitem{MBS-00}
M\"uller,~M.; Binder,~K.; Sch\"afer,~L. {\em Macromolecules} {\bf 2000},
 {\em 33}, 4568.


